Simulations of a bubble wall interacting with an electroweak plasma

We perform large-scale real-time simulations of a bubble wall sweeping through an out-of-equilibrium plasma. The scenario we have in mind is the electroweak phase transition, which may be first order in extensions of the Standard Model, and produce such bubbles. The process may be responsible for baryogenesis and can generate a background of primordial cosmological gravitational waves. We study thermodynamic features of the plasma near the advancing wall, the generation of Chern-Simons number/Higgs winding number and consider the potential for CP-violation at the wall generating a baryon asymmetry. A number of technical details necessary for a proper numerical implementation are developed.

==> bubble_aux.tex <==

%\cite{Coleman:1977py}
\bibitem{Coleman:1977py}
S.~R.~Coleman,
``The Fate of the False Vacuum. 1. Semiclassical Theory,''
Phys. Rev. D \textbf{15}, 2929-2936 (1977)
%doi:10.1103/PhysRevD.16.1248
%1995 citations counted in INSPIRE as of 13 May 2020


\section{Theory on a lattice:}


\begin{align}
{\mathcal L} &= \sum_i \frac{2}{(g_1dtdx_i)^2} \left(2-V_{0i} - V_{i0}\right) 
 -\sum_{ij}\frac{1}{(g_1dx_idx_j)^2} \left(2-V_{ij} - V_{ji}\right) 
\nonumber \\ & 
 + \sum_i \frac{4}{(g_2dtdx_i)^2} \left( 1- \frac{1}{2} {\rm Tr} U_{0i}\right) 
 - \sum_{ij} \frac{2}{(g_2dx_idx_j)^2} \left( 1- \frac{1}{2} {\rm Tr} U_{ij}\right) 
\nonumber \\ & 
 +\frac{1}{4} {\rm Tr} \left[ \dot \Phi^\dagger \dot \Phi \right]
 -\frac{1}{4} \sum_i {\rm Tr} \left[ (D_i \Phi)^\dagger (D_i \Phi) \right]
 -\frac{m_H^2}{2v^2}  \left(  \frac{1}{4} {\rm Tr} [ \Phi^\dagger\Phi ] - \frac{v^2}{2} \right)^2
\nonumber \\ & 
+\Delta {\mathcal L}
\end{align}
 

\begin{align}
U_\mu(x) &\sim \exp \left(-\frac{i\sigma^a}{2}g_2dx_\mu W^a_\mu(x) \right), \nonumber \\
V_\mu(x) &\sim \exp \left(\frac{i}{2}g_1dx_\mu B_\mu(x)\right),
\end{align}
\begin{align}
U_{\mu\nu}(x) &\sim \exp \left(-\frac{i\sigma^a}{2}g_2dx_\mu dx_\nu W^a_{\mu\nu} \right), \nonumber \\
V_{\mu\nu}(x) &\sim \exp \left(\frac{i}{2}g_1dx_\mu dx_\nu B_{\mu\nu}\right),
\end{align}

\begin{align}
Z_\mu(x)
=\left( \begin{array}{cc} V^*_{\mu}(x) & 0  \\  0 & V_{\mu}(x) \end{array}\right)
 &\sim \exp \left(-\frac{i\sigma^3}{2}g_1dx_\mu B_\mu(x)\right)
\end{align}


\begin{align}
~^1U^a_{\mu \nu}(x)  =&  {\rm Tr}\left[ i\sigma^a U_\mu(x)U_\nu(x+\mu)U^\dagger_\mu(x+\nu)U^\dagger_\nu(x) \right]
,\nonumber \\ 
~^2U^a_{\mu \nu}(x)  =&  {\rm Tr}\left[ U_\mu(x)i\sigma^a U_\nu(x+\mu)U^\dagger_\mu(x+\nu)U^\dagger_\nu(x) \right]
,\nonumber \\  
~^3U^a_{\mu \nu}(x)  =&  {\rm Tr}\left[ U_\mu(x)U_\nu(x+\mu)U^\dagger_\mu(x+\nu)i\sigma^a U^\dagger_\nu(x) \right]
,\nonumber \\ 
~^4U^a_{\mu \nu}(x)  =&  {\rm Tr}\left[ U_\mu(x)U_\nu(x+\mu)U^\dagger_\mu(x+\nu)U^\dagger_\nu(x)i\sigma^a  \right]
,
\end{align}

\begin{align}
~^1U^a_{\mu \nu}(x)  = ~^4U^a_{\mu \nu}(x)  =  -~^4U^{a}_{\nu \mu}(x)  
,\quad
~^2U^a_{\mu \nu}(x)  =  -~^3U^{a}_{\nu \mu}(x)  
.
\end{align}

\begin{align}
E_i \sim B_{i0}
,\quad
E_i^a \sim W_{i0}^a
\end{align}
\begin{align}
~^1U^a_{0i}(x) = -E_i^a(x)g_2dtdx_i = -~^1U^a_{i0}(x) 
\end{align}

\begin{align}
V_{0i}(x) - V_{i0}(x)  = -E_i(x)ig_1dtdx_i
\end{align}

\begin{align}
\overline E^a_i(x) = -\frac{1}{2} \sum_b{\rm Tr} \left[ i\sigma^a U^\dagger_i(x) i\sigma^b U_i(x) \right]E^b_i(x)
\end{align}

\begin{align}
~^2U^a_{0i}(x) = ~^1U^a_{0i}(x)
,\quad
~^2U^a_{i0}(x) = \overline E_i^a(x)g_2dtdx_i
\end{align}

\subsection{Equation of motion}


Higgs fields:
\begin{align}
\frac{\dot\Phi(x)-\dot\Phi(x-0)}{dt}& =
\sum_i \frac{U_i(x)\Phi(x+i) Z_i(x) -2\Phi(x) + U_i^\dagger(x-i) \Phi(x-i) Z_i^\dagger(x-i)}{d^2x_i}
\nonumber \\
&- \frac{m_H^2}{v^2} \left(\frac{1}{4}{\rm Tr}\left[\Phi^\dagger(x) \Phi(x)\right] - \frac{v^2}{2}\right) \Phi(x)
 +\sum_\beta\frac{\partial \Delta {\mathcal L_2}}{\partial \Phi_\beta}k_\beta
\end{align}
\begin{align}
\Phi(x+0) = \Phi(x)+dt\dot\Phi(x)
\end{align}


$U(1)$ gauge field:
\begin{align}
\hspace{-1cm}
\frac{E_{i}(x)-E_{i}(x-0)}{dt} =
- \sum_j\frac{i}{g_1dx_id^2x_j}\left[V_{ij}(x)-V_{ji}(x)+V_{ji}(x-j)-V_{ij}(x-j)\right]- j^{i}_{\Phi}  
\end{align}
\begin{align}
V_i(x+0) = \left[\sqrt{1-\left(\frac{g_1}{2}dtdx_iE_i(x)\right)^2} - i\frac{g_1}{2}dtdx_iE_i(x) \right] V_i(x)
\end{align}

$SU(2)$ gauge fields:
\begin{align}
\frac{E^a_{i}(x)-E^a_{i}(x-0)}{dt} &=
 \sum_j\frac{1}{g_2dx_id^2x_j}\left[~^1U^a_{ij}(x)+~^2U^a_{ji}(x-j)\right]  - J^{i,a}_{\Phi} - \frac{\partial \Delta {\mathcal L_2}}{\partial W^a_i}
\end{align}
\begin{align}
U_i(x+0) = \left[\sqrt{1-\sum_a\left(\frac{g_2}{2}dtdx_iE_i^a(x)\right)^2} + \sum_ai\sigma^a\frac{g_2}{2}dtdx_iE_i^a(x) \right] U_i(x)
\end{align}




\subsection{Currents}

\begin{align}
j_{\Phi}^i  = \left(- \frac{g_1}{4dx_i}\right) {\rm Tr} \left[ \Phi^\dagger(x) U_i(x) \Phi(x+i) Z_i(x) i\sigma^3  \right]
\end{align}

\begin{align}
J_{\Phi}^{i,a}  = \left(- \frac{g_2}{4dx_i} \right) {\rm Tr} \left[ \Phi^\dagger(x) i\sigma^a U_i(x)\Phi(x+i) Z_i(x) \right]
\end{align}

\subsection{Gauss law}
\begin{align}
\sum_i\frac{E_i(x)-E_i(x-i)}{dx_i} = \rho_\Phi + \rho_F+ \frac{\delta \Delta {\mathcal L_1}}{\delta B_0}
\end{align}

\begin{align}
\sum_i\frac{E^a_i(x)-\overline{ E}^a_{i}(x-i)}{dx_i} = \rho^{a}_\Phi + \rho^{a}_F + \frac{\delta \Delta {\mathcal L_2}}{\delta W^a_0}
\end{align}


\begin{align}
\rho_{\Phi}^0 &= \frac{g_1}{2} \left[
 \Phi^3 \dot\Phi^0
+\Phi^2 \dot\Phi^1
-\Phi^1 \dot\Phi^2
-\Phi^0 \dot\Phi^3
 \right] 
,\nonumber \\
\rho_{\Phi}^{1} &= \frac{g_2}{2} \left[
 \Phi^1 \dot\Phi^0
-\Phi^0 \dot\Phi^1
-\Phi^3 \dot\Phi^2
+\Phi^2 \dot\Phi^3
 \right] 
,\nonumber \\
\rho_{\Phi}^{2} &= \frac{g_2}{2} \left[
 \Phi^2 \dot\Phi^0
+\Phi^3 \dot\Phi^1
-\Phi^0 \dot\Phi^2
-\Phi^1 \dot\Phi^3
 \right] 
,\nonumber \\
\rho_{\Phi}^{3} &= \frac{g_2}{2} \left[
 \Phi^3 \dot\Phi^0
-\Phi^2 \dot\Phi^1
+\Phi^1 \dot\Phi^2
-\Phi^0 \dot\Phi^3
 \right] 
,
\end{align}




\subsection{CPT}

\begin{align}
\Phi(x) \rightarrow \Phi(-x)
,\quad
U_i(x) \rightarrow U^\dagger_i (-x-i)
\end{align}

For the $x$ associated with the site $(s_1,s_2,s_3)$, it is transformed into the site $(N_1-1-s_1,N_2-1-s_2,N_3-1-s_3)$.

charge conjugation:

\begin{align}
\Phi(x) \rightarrow \Phi^*(x)
,\quad
U_i(x) \rightarrow U^*_i (x)
\end{align}

Time reversal:


\begin{align}
\Phi(t,x) \rightarrow \Phi^*(-t,x)
,\quad
U_i(t,x) \rightarrow U^*_i (-t,x)
\end{align}


\subsection{Thermal Mass}


We consider the potential for the Higgs fields, including their interaction with gauge fields,
\begin{align}
V=\left|  \left(-i\frac{g_2^2}{2} \sigma^a W^a_i  +i\frac{g_1^2}{2} B_i \right) \phi \right|^2
+\frac{m_H^2}{2v^2} \left( \phi^\dagger \phi -\frac{v^2}{2} \right)^2
+J\phi^\dagger\phi,
\end{align}
where the external current $J$ is treated as a constant in the initialization, not depending on time or space.
We assume the real components of the Higgs fields initially satisfy the correlation,
\begin{align}
\Big\langle \Phi^\dagger_m(p) \Phi_n(p') \Big\rangle = \delta_{mn} \frac{n_{\Phi}(p)}{\omega_{\Phi}(p)}(2\pi)^3\delta^3(p-p'),
\end{align}
and similarly, for gauge fields
\begin{align}
\Big\langle W^{a,\dagger}_i(p) W^b_j(p')\Big \rangle &= \delta^{ab} \frac{n_{W}(p)}{\omega_{W}(p)}\left(\delta_{ij}-\frac{p_ip_j}{p^2}\right)(2\pi)^3\delta^3(p-p'),
\\
\Big\langle B^\dagger_i(p) B_j(p')\Big \rangle &=  \frac{n_{B}(p)}{\omega_{B}(p)}\left(\delta_{ij}-\frac{p_ip_j}{p^2}\right)(2\pi)^3\delta^3(p-p'),
\end{align}
where $n$ and $\omega$ are the particle number and energy for related fields.
We also assume any other correlations vanish initially, and therefore cross terms can be ignored in the following calculation.
The potential then admits a simple form, 
\begin{align}
V=\frac{1}{2} \left(\sum_n \Phi_n^2 \right) 
\left( \frac{g_2^2}{4}\sum_{i,a} W_i^a W_i^a +\frac{g_1^2}{4}\sum_i B_i B_i\right) 
+\frac{m_H^2}{8v^2} \left( \sum_n \Phi^2_n -v^2  \right)^2
+\frac{J}{2} \sum_n \Phi^2_n.
\end{align}
We can derive the effective mass of Higgs fields through derivative of the potential,
\begin{align}
&m^2_{\Phi} = \Bigg\langle \frac{\delta^2 V}{\delta (\Phi_n)^2} \Bigg\rangle
\nonumber \\
=&\frac{g_2^2}{4}\sum_{i,a} \Big\langle W_i^a W_i^a \Big\rangle +\frac{g_1^2}{4}\sum_i \Big\langle  B_i B_i \Big\rangle 
+\frac{m_H^2}{8v^2} \left( 12\Big\langle \Phi^2_n\Big\rangle  -4v^2  + 4 \sum_{m\neq n} \Big\langle \Phi_m^2\Big\rangle  \right)
+J
\nonumber \\
=&\frac{6g_2^2}{4}\Big\langle W^2\Big\rangle+\frac{2g_1^2}{4} \Big\langle  B^2 \Big\rangle 
+\frac{6m_H^2}{2v^2} \Big\langle \Phi^2\Big\rangle
+J-\frac{m_H^2}{2}  
\nonumber \\
=&\frac{g_2^2}{8}T^2+\frac{g_1^2}{24}T^2+\frac{6m_H^2}{2v^2} \Big\langle \Phi^2\Big\rangle
+J-\frac{m_H^2}{2} ,
\label{eq:mass}
\end{align}
with abbreviations standing for,
\begin{align}
\label{Phi}
&\Big\langle\Phi^2 \Big\rangle = \int \frac{d^3p}{(2\pi)^3} \frac{n_{\Phi}(p)}{\omega_{\Phi}(p)}
,\quad \omega_{\Phi}(p)=\sqrt{p^2+m^2_\Phi}
,\quad n_{\Phi}(p)=\frac{1}{e^{\frac{\omega_{\Phi}(p)}{T}}-1},
\nonumber \\
&\Big\langle W^2 \Big\rangle = \int \frac{d^3p}{(2\pi)^3} \frac{n_{W}(p)}{\omega_{W}(p)}=\frac{T^2}{12}
,\quad \omega_{W}(p)=p
,\quad n_{W}(p)=\frac{1}{e^{\frac{\omega_{W}(p)}{T}}-1},
\nonumber \\
&\Big\langle B^2 \Big\rangle = \int \frac{d^3p}{(2\pi)^3} \frac{n_{B}(p)}{\omega_{B}(p)}=\frac{T^2}{12}
,\quad \omega_{B}(p)=p
,\quad n_{B}(p)=\frac{1}{e^{\frac{\omega_{B}(p)}{T}}-1}.
\end{align}
The thermal mass is equal for all four Higgs real components and can be obtained by the derivative with respect to any of them. 
In the above calculation, we consider only two transverse modes of each gauge boson and do not attribute thermal mass to them.
\Cref{eq:mass} is an implicit equation, as $\langle \Phi^2\rangle$ also depends on the thermal mass $m^2_{\Phi}$.
But given temperature $T$, one can solve \cref{eq:mass} numerically by recurrence method.

